Multilevel decompositions and norms for negative order Sobolev spaces

We consider multilevel decompositions of piecewise constants on simplicial meshes that are stable in $H^{-s}$ for $s\in (0,1)$. Proofs are given in the case of uniformly and locally refined meshes. Our findings can be applied to define local multilevel diagonal preconditioners that lead to bounded condition numbers (independent of the mesh-sizes and levels) and have optimal computational complexity. Furthermore, we discuss multilevel norms based on local (quasi-)projection operators that allow the efficient evaluation of negative order Sobolev norms. Numerical examples and a discussion on several extensions and applications conclude this article.

==> MLN.tex <==
\begin{tikzpicture}
\begin{loglogaxis}[
    title={$s=\tfrac12$},
%height=7cm,
width=0.49\textwidth,
%cycle list name=black white,
%cycle list name=exotic,
cycle list/Dark2-6,
% combine it with ’mark list*’:
cycle multiindex* list={
mark list*\nextlist
Dark2-6\nextlist},
every axis plot/.append style={ultra thick},
xlabel={number of elements $\#\TT$},
%ylabel={errors and estimators},
grid=major,
legend entries={\small $\lambda_{\mathrm{max},\projHone'}$,\small $\lambda_{\mathrm{min},\projHone'}$,\small $\lambda_{\mathrm{max},\projLtwo}$,\small $\lambda_{\mathrm{min},\projLtwo}$},
legend pos=south west,
]
\addplot table [x=nE,y=maxB] {MLNs12.dat};
\addplot table [x=nE,y=minB] {MLNs12.dat};
\addplot table [x=nE,y=maxL2] {MLNs12.dat};
\addplot table [x=nE,y=minL2] {MLNs12.dat};
\end{loglogaxis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{loglogaxis}[
    title={$s=\tfrac34$},
%height=7cm,
width=0.49\textwidth,
%cycle list name=black white,
%cycle list name=exotic,
cycle list/Dark2-6,
% combine it with ’mark list*’:
cycle multiindex* list={
mark list*\nextlist
Dark2-6\nextlist},
every axis plot/.append style={ultra thick},
xlabel={number of elements $\#\TT$},
%ylabel={errors and estimators},
grid=major,
legend entries={\small $\lambda_{\mathrm{max},\projHone'}$,\small $\lambda_{\mathrm{min},\projHone'}$,\small $\lambda_{\mathrm{max},\projLtwo}$,\small $\lambda_{\mathrm{min},\projLtwo}$},
legend pos=south west,
]
\addplot table [x=nE,y=maxB] {MLNs34.dat};
\addplot table [x=nE,y=minB] {MLNs34.dat};
\addplot table [x=nE,y=maxL2] {MLNs34.dat};
\addplot table [x=nE,y=minL2] {MLNs34.dat};
\end{loglogaxis}
\end{tikzpicture}


==> condAdap.tex <==
\begin{tikzpicture}
\begin{loglogaxis}[
%    title={$s=0$},
%height=7cm,
width=0.49\textwidth,
%cycle list name=black white,
%cycle list name=exotic,
cycle list/Dark2-6,
% combine it with ’mark list*’:
cycle multiindex* list={
mark list*\nextlist
Dark2-6\nextlist},
every axis plot/.append style={ultra thick},
xlabel={number of elements $\#\TT$},
%ylabel={errors and estimators},
grid=major,
legend entries={\small $\kappa(\Cmat_0^{-1}\Hmat_{0})$,\small $\kappa(\Pmat_{0}^{-1}\Hmat_{0})$,\small $\kappa(\Cmat_{1/4}^{-1}\Hmat_{-1/4})$,\small $\kappa(\Pmat_{1/4}^{-1}\Hmat_{-1/4})$},
%legend pos=north west,
%legend pos=outer north east
legend style={at={(0.5,1.05)},anchor=south},
legend columns=2, 
        legend style={
                    % the /tikz/ prefix is necessary here...
                    % otherwise, it might end-up with `/pgfplots/column 2`
                    % which is not what we want. compare pgfmanual.pdf
            /tikz/column 2/.style={
                column sep=5pt,
            }},
]
\addplot table [x=nE,y=condD] {cond0adap.dat};
\addplot table [x=nE,y=condP] {cond0adap.dat};
\addplot table [x=nE,y=condD] {cond14adap.dat};
\addplot table [x=nE,y=condP] {cond14adap.dat};

\end{loglogaxis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{loglogaxis}[
%    title={$s=0$},
%height=7cm,
width=0.49\textwidth,
%cycle list name=black white,
%cycle list name=exotic,
cycle list/Set1-5,
% combine it with ’mark list*’:
cycle multiindex* list={
mark list*\nextlist
Set1-5\nextlist},
every axis plot/.append style={ultra thick},
xlabel={number of elements $\#\TT$},
%ylabel={errors and estimators},
grid=major,
legend entries={\small $\kappa(\Cmat_{1/2}^{-1}\Hmat_{-1/2})$,\small $\kappa(\Pmat_{1/2}^{-1}\Hmat_{-1/2})$,\small $\kappa(\Cmat_{3/4}^{-1}\Hmat_{-3/4})$,\small $\kappa(\Pmat_{3/4}^{-1}\Hmat_{-3/4})$},
%legend pos=north west,
%legend pos=outer north east
legend style={at={(0.5,1.05)},anchor=south},
legend columns=2, 
        legend style={
                    % the /tikz/ prefix is necessary here...
                    % otherwise, it might end-up with `/pgfplots/column 2`
                    % which is not what we want. compare pgfmanual.pdf
            /tikz/column 2/.style={
                column sep=5pt,
            }},
]
\addplot table [x=nE,y=condD] {cond12adap.dat};
\addplot table [x=nE,y=condP] {cond12adap.dat};
\addplot table [x=nE,y=condD] {cond34adap.dat};
\addplot table [x=nE,y=condP] {cond34adap.dat};

\end{loglogaxis}
\end{tikzpicture}


==> condUnif.tex <==
\begin{tikzpicture}
\begin{loglogaxis}[
%    title={$s=0$},
%height=7cm,
width=0.49\textwidth,
%cycle list name=black white,
%cycle list name=exotic,
cycle list/Dark2-6,
% combine it with ’mark list*’:
cycle multiindex* list={
mark list*\nextlist
Dark2-6\nextlist},
every axis plot/.append style={ultra thick},
xlabel={number of elements $\#\TT$},
%ylabel={errors and estimators},
grid=major,
legend entries={\small $\kappa(\Cmat_0^{-1}\Hmat_{0})$,\small $\kappa(\Pmat_{0}^{-1}\Hmat_{0})$,\small $\kappa(\Cmat_{1/4}^{-1}\Hmat_{-1/4})$,\small $\kappa(\Pmat_{1/4}^{-1}\Hmat_{-1/4})$},
%legend pos=north west,
%legend pos=outer north east
legend style={at={(0.5,1.05)},anchor=south},
legend columns=2, 
        legend style={
                    % the /tikz/ prefix is necessary here...
                    % otherwise, it might end-up with `/pgfplots/column 2`
                    % which is not what we want. compare pgfmanual.pdf
            /tikz/column 2/.style={
                column sep=5pt,
            }},
]
\addplot table [x=nE,y=condD] {cond0unif.dat};
\addplot table [x=nE,y=condP] {cond0unif.dat};
\addplot table [x=nE,y=condD] {cond14unif.dat};
\addplot table [x=nE,y=condP] {cond14unif.dat};

\end{loglogaxis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{loglogaxis}[
%    title={$s=0$},
%height=7cm,
width=0.49\textwidth,
%cycle list name=black white,
%cycle list name=exotic,
cycle list/Set1-5,
% combine it with ’mark list*’:
cycle multiindex* list={
mark list*\nextlist
Set1-5\nextlist},
every axis plot/.append style={ultra thick},
xlabel={number of elements $\#\TT$},
%ylabel={errors and estimators},
grid=major,
legend entries={\small $\kappa(\Cmat_{1/2}^{-1}\Hmat_{-1/2})$,\small $\kappa(\Pmat_{1/2}^{-1}\Hmat_{-1/2})$,\small $\kappa(\Cmat_{3/4}^{-1}\Hmat_{-3/4})$,\small $\kappa(\Pmat_{3/4}^{-1}\Hmat_{-3/4})$},
%legend pos=north west,
%legend pos=outer north east
legend style={at={(0.5,1.05)},anchor=south},
legend columns=2, 
        legend style={
                    % the /tikz/ prefix is necessary here...
                    % otherwise, it might end-up with `/pgfplots/column 2`
                    % which is not what we want. compare pgfmanual.pdf
            /tikz/column 2/.style={
                column sep=5pt,
            }},
]
\addplot table [x=nE,y=condD] {cond12unif.dat};
\addplot table [x=nE,y=condP] {cond12unif.dat};
\addplot table [x=nE,y=condD] {cond34unif.dat};
\addplot table [x=nE,y=condP] {cond34unif.dat};

\end{loglogaxis}
\end{tikzpicture}

